The Effect of Behavioral Probability Weighting in a Simultaneous Multi-Target Attacker-Defender Game

We consider a security game in a setting consisting of two players (an attacker and a defender), each with a given budget to allocate towards attack and defense, respectively, of a set of nodes. Each node has a certain value to the attacker and the defender, along with a probability of being successfully compromised, which is a function of the investments in that node by both players. For such games, we characterize the optimal investment strategies by the players at the (unique) Nash Equilibrium. We then investigate the impacts of behavioral probability weighting on the investment strategies; such probability weighting, where humans overweight low probabilities and underweight high probabilities, has been identified by behavioral economists to be a common feature of human decision-making. We show via numerical experiments that behavioral decision-making by the defender causes the Nash Equilibrium investments in each node to change (where the defender overinvests in the high-value nodes and underinvests in the low-value nodes).

==> Related_Work.tex <==
\section{Related Work}\label{sec:lit-review}

 Game theory has been used to describe the interactions between attackers and defenders and their effects on CPS system security. A commonly used model in this context is that of two-player games, where a single attacker attempts to compromise a system controlled by a single defender \cite{guan2017modeling, roy2010survey}. In this context, simultaneous move games (where the defender and attacker allocate resources simultaneously) and Stackelberg games (where the defender plays the role
of the leader and the adversary acts as the follower) have been frequently studied (see the seminal papers ~\cite{pita2008deployed,yin2010stackelberg}). Specifically, the recent work \cite {guan2017modeling} considered such games for Multi-Target security with budget constraints.
  
Game theoretic models for the study of CPS security have been proposed in~\cite{ferdowsi2017colonel,perelman2014network,zhu2011stackelberg,9095996}. The problem of security resource allocation for smart city infrastructures was studied in \cite{ferdowsi2017colonel} as a Colonel Blotto game. The work in \cite{perelman2014network} proposed a single-defender game-theoretic approach to minimize loss due to attacks in water distribution networks. 
The authors in \cite{zhu2011stackelberg} proposed
a Stackelberg game model, in which a defender attempts to maintain high performance in a SCADA control system against cyber attacks launched by fully rational jammers. The work in~\cite{9095996} has proposed two-player Stackelberg semi-Markov games for modelling the strategic interactions between Dynamic Information Flow Tracking (DIFT) and advanced persistent threats (APT). 

The major difference of our work with all aforementioned literature is that existing work has focused on classical game-theoretic models of rational decision-making, while we analyze behavioral models of decision-making and its effect on the investment decisions. Notable exceptions from classical game-theoretic models of rational decision-making are~\cite{9030279,sanjab2017prospect,7544460,abdallah2019impacts}; however, these exceptions have either focused on the impact of probability weighting on a single defender's decisions via decision-theoretic analysis (with no strategic attacker)~\cite{9030279}, on multiple defenders' investments in networks (with the emphasis being on understanding the role of the network structure)~\cite{7544460,abdallah2019impacts}, or on behavioral decision-making by both players for settings with a single target  \cite{sanjab2017prospect}. In contrast to these works, we consider the effects of behavioral decision-making in a setting with multiple targets with different values to the players (i.e., the defender and the attacker). 

%\noindent \textbf{Human behavior in security of CPS:}
A different line of previous work in the literature has studied the effect of behavioral decision-making via psychological studies~\cite{anderson2012security} (see \cite{anderson2007information} for a survey), and human subject experiments~\cite{redmiles2018dancing,baddeley2011information}.
Our work differs from these lines of work in that we explore a rigorous mathematical framework for analyzing the players' behavior, and specifically investigate the interaction between defender and attacker when the CPS assets have heterogeneous valuations. This setting is useful for modelling  different CPS scenarios. 

